Constraints on the Galactic Population of TEV Pulsar Wind Nebulae Using Fermi Large Area Telescope Observations

Pulsar wind nebulae (PWNe) have been established as the most populous class of TeV gamma-ray emitters. Since launch, the Fermi Large Area Telescope (LAT)identified five high-energy (100MeV <E< 100 GeV) gamma-ray sources as PWNe, and detected a large number of PWNe candidates, all powered by young and energetic pulsars. The wealth of multi-wavelength data available and the new results provided by Fermi-LAT give us an opportunity to find new PWNe and to explore the radiative processes taking place in known ones. The TeV gamma-ray unidentifiedsources (UNIDs) are the best candidates for finding new PWNe. Using 45 months of Fermi-LAT data for energies above 10 GeV, an analysis was performed near the position of 58TeV PWNe and UNIDs within 5deg of the Galactic Plane to establish new constraints on PWNe properties and find new clues on the nature of UNIDs. Of the 58 sources, 30 were detected, and this work provides their gamma-rayfluxes for energies above 10 GeV. The spectral energy distributions (SED) andupper limits, in the multi-wavelength context, also provide new information on the source nature and can help distinguish between emission scenarios, i.e. between classification as a pulsar candidate or as a PWN candidate. Six new GeV PWNe candidates are described in detail and compared with existing models. A population study of GeV PWNe candidates as a function of the pulsar/PWN system characteristics is presented.

==> Makefile <==
manuscript = pwncat2

# These commands make sure no compression is applied
# when running ps2pdf
# http://cosmocoffee.info/viewtopic.php?p=213
PS2PDFARGS = "-dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode"

DEFBWFIGS = \def\bwfigures{true}

color: $(manuscript).pdfcolor

bw: $(manuscript).pdfbw


%.pdfcolor: %.dvicolor
	dvips $(manuscript)
	ps2pdf ${PS2PDFARGS} $(manuscript).ps

%.pdfbw: %.dvibw
	dvips $(manuscript)
	ps2pdf ${PS2PDFARGS} $(manuscript).ps

%.dvibw: %.tex
	latex "${DEFBWFIGS} \input{$(manuscript)}"
	bibtex $(manuscript) 
	latex "${DEFBWFIGS} \input{$(manuscript)}"
	latex "${DEFBWFIGS} \input{$(manuscript)}"

%.dvicolor: %.tex
	latex $(manuscript).tex
	bibtex $(manuscript) 
	latex $(manuscript).tex
	latex $(manuscript).tex

clean:
	-rm -f $(manuscript).aux $(manuscript).log $(manuscript).out \
      $(manuscript).toc $(manuscript).dvi $(manuscript).bbl \
      $(manuscript).blg $(manuscript).ps $(manuscript).tdo


